Digraph Decompositions and Monotonicity in Digraph Searching

We consider monotonicity problems for graph searching games. Variants of these games - defined by the type of moves allowed for the players - have been found to be closely connected to graph decompositions and associated width measures such as path- or tree-width. Of particular interest is the question whether these games are monotone, i.e. whether the cops can catch a robber without ever allowing the robber to reach positions that have been cleared before. The monotonicity problem for graph searching games has intensely been studied in the literature, but for two types of games the problem was left unresolved. These are the games on digraphs where the robber is invisible and lazy or visible and fast. In this paper, we solve the problems by giving examples showing that both types of games are non-monotone. Graph searching games on digraphs are closely related to recent proposals for digraph decompositions generalising tree-width to directed graphs. These proposals have partly been motivated by attempts to develop a structure theory for digraphs similar to the graph minor theory developed by Robertson and Seymour for undirected graphs, and partly by the immense number of algorithmic results using tree-width of undirected graphs and the hope that part of this success might be reproducible on digraphs using a directed tree-width. Unfortunately the number of applications for the digraphs measures introduced so far is still small. We therefore explore the limits of the algorithmic applicability of digraph decompositions. In particular, we show that various natural candidates for problems that might benefit from digraphs having small directed tree-width remain NP-complete even on almost acyclic graphs.

==> furtherresearch.tex <==
\section{Conclusion and Open Problems}
\label{sec:conclusion}

In this paper we considered graph searching games on directed graphs
and established non-monotonicity for two important types of games. Our
examples show that the monotonicity costs for these games can not be
bound by an additive term, i.e.~for any $k$ there are digraphs where
at least $k$ additional cops are required to catch a robber with a
monotone strategy. However, so far there is no upper bound for the
monotonicity costs involved. It is conceivable that there is a
constant $c\in\N$ such that whenever $n$ cops suffice to catch a
robber on a digraph $D$ in any of the two variants, than $c\cdot n$ cops
suffice for a monotone strategy. This, however, is left as an open problem.

A different trait we explored in this paper are the limits of an
algorithm theory based on directed graph decompositions. We showed that while there are
interesting and important examples for natural problems that become
tractable on digraphs of small width, many other natural problems
remain NP-complete even if the digraphs have very low global connectivity.

% We remark, though, that our results are within the
% framework of classical complexity. In particular, our results do rule
% out that problems such as the directed feedback vertex set problem are
% fixed-parameter tractable. However, our results suggest that 
% such a proof may not rely on directed graph
% decompositions. A study of the
% parameterized complexity in relation to directed tree-width is left
% for future work.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "soda"
%%% End: 


==> introduction.tex <==
\section{ Introduction }
\label{introduction}


The seminal work of Robertson and Seymour in their graph minor
project has focused much attention on graph decompositions and
associated measures of graph connectivity such as tree- or path- width.
Aside from the interest in graph structure theory,
these notions have also proved fruitful in the development of
algorithms. The tree-width of a graph is a measure of how tree-like the
graph is and small tree-width allows for graph
decompositions along which recursive algorithms can work. Many
problems that are intractable in general can be solved efficiently on
graphs of bounded tree-width. These include such classical NP-complete
problems as finding a Hamiltonian-cycle in a graph or detecting if a
graph is three-colourable. See \cite{bodlaender98,Bod97} and
references therein for an introduction to tree-width.

%\noindent\textbf{Digraph search games. }
Closely related to the theory of graph decompositions is the theory of
graph searching games. In a graph searching
game a number of searchers, or cops,
tries to catch a fugitive, or robber, hiding in the graph. 
There are many variants of these games. The robber can hide on edges
or vertices, he can be fast or lazy, he can be visible or not, the
game can be played on undirected or directed graphs, and many more.
Graph searching games are particularly interesting in relation to
graph decompositions, as many width measures for graphs based on
decompositions can also be described in terms of variants of Cops and
Robber games. For instance, in 1993, Seymour and Thomas \cite{ST93}
showed that the tree-width of a 
graph equals 
the minimal number of cops required to catch a visible and fast robber
(minus one). Dendris, Kirousis, and Thilikos \cite{DendrisKirThi97} gave
an analogous characterisation in terms of an invisible, lazy robber game.
Other variants of Cops and Robber games have also been used to
characterise the path-width of graphs and similar connectivity
measures. 

An important concept in the theory of graph searching games is
monotonicity. A game is \emph{monotone}, if whenever $k$ cops can
catch a robber on a graph they can do so without allowing the robber
to re-occupy vertices. In general, restricting
the cops to monotone strategies may require additional cops to catch a
robber. LaPaugh \cite{LaPaugh93} gave a first proof
of monotonicity for a Cops and Robber game. Since then, monotonicity
has been intensely studied  
and a large number of monotonicity results have been established. See
e.g.~\cite{LaPaugh93,BienstockSey91,DendrisKirThi97,Bar04,Dyer04,FominThi01,MazoitNis07,YangC07}
or the survey \cite{Alspach04} and references therein.

% Concerning games played on directed graphs, Bar\'{a}t \cite{Bar04} showed that the
% invisible, fast Cops and Robber game is monotone on digraphs and corresponds
% to a directed analogue of path-width. On the other hand, Johnson et
% al. \cite{JRST01} and Adler \cite{Adler05} established non-monotonicity
% for two types of monotonicity (see below) in the Cops and Robber game
% corresponding to the directed tree-width 
% introduced by Johnson, Robertson, Seymour, and Thomas in \cite{JRST01}. 
% In Section~\ref{sec:decomp}, we resolve the case for
% \emph{robber-monotonicity} by showing 
% that the monotonicity
% costs for robber-monotone strategies in this game are bounded by a
% factor of $3$ (plus a small additive term).

Despite the considerable interest and the large number of results in
this field, two cases have so far resisted any attempts to solve the
monotonicity problem -- the Cops and Robber game with a visible, fast
robber and the game with an invisible, lazy robber, both played on digraphs.
%It is these games that are closely related to DAG- and
%Kelly-decompositions. 
In this paper,we solve the problems by showing that both
games are non-monotone. 

\medskip

\noindent\textbf{Digraph decompositions. } In recent years, attempts
have been made to generalise the notion of tree-decompositions and
their algorithmic applications  to directed
graphs. 
Clearly, we can define the tree-width of a directed graph as the tree-width
of the undirected graph
we get by forgetting the direction of edges, a process which leads to
some loss of information.  This loss may be significant, if the
algorithmic problems we are interested in are inherently directed.  A
good example is the problem of detecting Hamiltonian cycles.  While we
know that this can be solved easily on graphs with small tree-width,
there are directed graphs with very simple connectivity structure
which have large tree-width.  Therefore, several proposals have been made to 
extend the notions of tree-decompositions and tree-width to directed
graphs (see 
\cite{MR1966425,JRST01,Bar04,BG04,Saf05,HunterKre07}).  In particular, Reed \cite{MR1966425} and Johnson, Robertson, Seymour, and
Thomas~\cite{JRST01} introduce the 
notion of \emph{directed tree-width} and they show that Hamiltonicity
can be solved for graphs 
of bounded directed tree-width in polynomial time. 

Following this initial paper, several alternative definitions of
directed graph decompositions have been proposed, with the aim of
overcoming some shortcomings of the original
definition. Obdr\v{z}\`{a}lek \cite{Obdrzalek06} and Berwanger, Dawar,
Hunter, and Kreutzer \cite{bdhk06} introduce the notion of DAG-width
and Hunter and Kreutzer \cite{HunterKre07} introduce the notion of
Kelly-width. 
All three proposals are supported by algorithmic applications and
various equivalent characterisations in terms 
of obstructions, elimination orderings, and, in particular,
variants of Cops and Robber games on directed graphs. 
However, so far the algorithmic applications are restricted to few
classes of problems, in particular the problem of finding disjoint
paths, Hamiltonian-cycles, and similar linkage problems and certain
problems in relation to combinatorial games (parity games) played on graphs that are
motivated by the theory of computer-aided verification. Whereas the
tree-width of undirected graphs has been employed to solve a huge number
of problems on graphs of small tree-width, the algorithmic theory of
directed graph decompositions is not nearly as rich. 

It is an obvious question whether this is due to the
fact that digraph decompositions are a relatively new field of
research, where the fundamental machinery first needs to be developed,
or whether this is due to a general limitation of this approach to
algorithms on digraphs. 
In this paper we systematically explore the range of algorithmic
applicability of digraph decompositions. For this, we look at
typical NP-complete problems on graphs -- as they can be found in
\cite{gareyjohnson79} for instance -- and 
identify those that are ``suitable''for this approach, 
where by ``suitable'' 
we mean that the problems should be NP-complete in general but be
tractable on acyclic graphs. The reason for the latter is that all
digraph decompositions proposed so far measure in some way the
similarity of a graph to being acyclic. In particular, acyclic graphs
have small width in all of these measures. Hence, if a problem
is already hard on acyclic digraphs, there is no point in studying the
effect of digraph decompositions on this problem. 
We then identify representatives for the
various types of ``suitable'' problems and ask whether they can be
solved in polynomial time on graphs of small directed tree-width,
Kelly- or DAG-width, or directed path-width.

The results we present in Section~\ref{sec:algorithms}
show that the border for algorithmic applicability of digraph
decompositions is rather tight. 
Essentially, as far as classical graph theoretical problems are concerned,
disjoint paths and Hamiltonian-cycles can be detected efficiently on graphs of small
directed tree-width, but all other problems we considered such as 
Minimum Equivalent Subgraph, Feedback Vertex Set (FVS), Feedback Arc Set,
Graph Grundy Numbering, and several others are NP-complete even on
graphs with a very low global connectivity and thus very low directed
path or tree-width.

% The NP-completeness result for directed FVS is particularly
% interesting as the problem whether the 
% directed FVS problem is fixed-parameter tractable  is an
% important open problem in fixed-parameter algorithms and there
% was hope that digraph decompositions might be useful to design an FPT
% algorithm for this problem. Although our result does not imply that
% there is no such algorithm, it casts doubt on whether directed
% tree-width or similar measures might be particularly useful to design
% such an algorithm.

\smallskip


\noindent\textbf{Organisation. } The paper is organised as follows. In
Section~\ref{sec:preliminaries} we briefly recall basic notions from
graph and game theory needed in the sequel. In Section~\ref{sec:games}
we give a formal description of Cops and Robber games and present the
first main result of this paper, the non-monotonicity of the two types
of games mentioned above. 
%In Section~\ref{sec:decomp} we introduce the
%concept of directed tree-width, give an alternative definition to
%overcome some issues with the original definition, and prove some
%basic results. 
In Section~\ref{sec:algorithms} we explore the algorithmic boundaries
of the digraph decompositions obtained so far by showing NP-completeness
for a number of problems on digraphs with bounded ``width''. 
We conclude and state some
open problems in Section~\ref{sec:conclusion}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "soda"
%%% End: 


==> preliminaries.tex <==
\section{ Preliminaries }
\label{sec:preliminaries}

We use standard notation from graph theory 
as can be found in, e.g.,~\cite{MR2159259}. 
All graphs and directed graphs in this work
 are finite and simple. 

Let $G$ be a (directed) graph. We denote the vertexset of $G$
by $V(G)$ and the edgeset of $G$ by $E(G)$. For 
$X \subseteq V(G)$ we denote by $G[X]$ the subgraph of
$G$ induced by $X$ and by $G \setminus X$ the subgraph of
$G$ induced by $V(G) \setminus X$. Similarly for $Y \subseteq E(G)$
we set $G \setminus Y$ to be the subgraph of $G$ after deleting all edges in 
$Y$. A path in $G$ from a vertex $v_{1}$ to a vertex $v_{n}$
is a subgraph of $G$ with vertices $v_{1}, \cdots, v_{n}$ 
and edges $\{\{v_{i},v_{i+1}\} \mid 1 \leq i < n\}$
if $G$ is undirected, respectively $\{(v_{i},v_{i+1}) \mid 1 \leq i < n\}$ if $G$ is
directed. For convenience we write $v \rightarrow u$ in $G$ if $G$ contains a path 
from $v$ to $u$. A cycle in $G$ is a path from $v_{1}$ to $v_{n}$ together
with an edge $\{v_{n},v_{1}\}$ if $G$ is undirected, and $(v_{n},v_{1})$ if $G$
is directed. We say $X \subseteq V(G)$ is connected, if for all
pairs $x,y \in X$ there is a path from $x$ to $y$ in $G[X]$. 
A component in $G$ is a maximal connected vertexset in $G$.

Finally, for a set $X$ and $k \in \N$, we denote by $[X]^{\leq k}$ the set of all
subsets of $X$ of cardinality $\leq k$.
% and by $[X]$ the powerset of $X$. 


%

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "soda"
%%% End: 

